Longhorn: State Space Models are Amortized Online Learners

Modern large language models are built on sequence modeling via next-token prediction. While the Transformer remains the dominant architecture for sequence modeling, its quadratic decoding complexity in sequence length poses a major limitation. State-space models (SSMs) present a competitive alternative, offering linear decoding efficiency while maintaining parallelism during training. However, most existing SSMs rely on linear recurrence designs that appear somewhat ad hoc. In this work, we explore SSM design through the lens of online learning, conceptualizing SSMs as meta-modules for specific online learning problems. This approach links SSM design to formulating precise online learning objectives, with state transition rules derived from solving these objectives. Based on this insight, we introduce a novel deep SSM architecture, Longhorn, whose update resembles the closed-form solution for solving the online associative recall problem. Our experimental results show that Longhorn outperforms state-of-the-art SSMs, including the Mamba model, on standard sequence modeling benchmarks, language modeling, and vision tasks. Specifically, Longhorn achieves a 1.8x improvement in sample efficiency compared to Mamba, and can extrapolate over contexts that are up to 16x longer during inference.

==> content/method_backup.tex <==
\section{An Online Learning Perspective For Sequence Mixing}
\label{sec::method}
As demonstrated in the previous section, designing a state-space model (SSM) depends on the specific selection of $(A_t, B_t, *)$, which is intricate and somewhat artisanal. In this section, we propose to streamline SSM design through an online learning perspective. The main idea is to treat the SSM layers as learning modules that learn to compress information along the sequence dimension. From this perspective, the SSM layers are \emph{learning to learn}, such that during the inference time, these layers are still learning (compressing) new information online.  

We begin with an overview of online learning and subsequently demonstrate how SSM can be framed as an online learning problem. Finally, we present a straightforward architecture based on the closed-form solution of the implicit online learning algorithm.

\subsection{SSM as Online Learning}
We advocate viewing the recurrence of SSM as solving an online learning problem. 
In online learning, the agent picks a state $s_t$ at time $t$ and then incurs a loss $\ell_t(s_t)$. The goal is to minimize
\begin{equation}
\min_{\{s_t\}} \sum_t \ell_t(s_t).
\label{eq:ocp-1}
\end{equation}
For instance, consider online linear prediction, where at each step the agent is given an input-label pair $(x_t, y_t)$ and $\ell_t(s_t) = \frac{1}{2}||s_t^\top x_t - y_t||^2$ is the $\ell_2$ regression loss, then the problem becomes an online regression problem, and the goal is to successfully predict $y_t$ given $x_t$ at future time steps, with the key feature that the prediction ($s_t$) can change with each new data point. 

Online convex programming (OCP) yields a principled approach to 
solving \Eqref{eq:ocp-1} when $\ell_t$ are convex, by trading-off the ``stability" and ``plasticity"~\citep[e.g.,][]{mermillod2013stability}. Formally, an online convex programming algorithm updates $s_t$ by 
solving a regularized cost function:
\begin{equation}
s_{t} = \argmin_s L_t(s),  ~~~~~~~ 
L_t(s) = \underbrace{D_\phi(s, s_{t-1})}_{\text{stability}} + \underbrace{\beta_t \ell_t(s)}_{\text{plasticity}},
\label{eq:ocp-stability-plasticity}
\end{equation}
where $\beta_t \in \RR^+$ and
$D_\phi$ is a discrepancy measure, often a Bregman divergence induced by the convex function $\phi$ (e.g., when $\phi(x) =  \frac{1}{2}\norm{x}^2$, $D_\phi(s, s_{t-1}) = \frac{1}{2}||s - s_{t-1}||^2$).
Here the first term ensures the updated $s$ will be close to the previous $s_{t-1}$, so the agent suffers less from \emph{catastrophic forgetting}, while the second term ensures the agent is incorporating new knowledge from minimizing the new loss $\ell_t(s)$. Hence, $\beta_t$ controls the trade-off between stability and plasticity.

\subsection{The \ours{} Architecture}

Under the online learning framework, the \textbf{design of an SSM reduces to the design of $D_\phi$ and $\ell_t$} in \Eqref{eq:ocp-stability-plasticity}. 
 This provides a unified framework for the existing SSM variants. 
We summarize in Table~\ref{tab:ssms} in Appendix~\ref{sec::apx-tab-ssms} the online learning interpretation of several existing SSM architectures. 

In this work, we explore a highly simplified and natural design called   \emph{Longhorn} guided by the online principle (see the last row of Table~\ref{tab:ssms}).    
%Guided by the principle 
In particular, we consider $\{(k_t, x_t)\}_t$ as the input stream, where $k_t \in \RR^m$ and $x_t \in \RR$ are the key-value pairs, just as in the Transformer model~\citep{vaswani2017attention}. In practice, as in Mamba~\citep{gu2023mamba}, $x_t \in \R^d$ is often a vector and $k_t = W_k x_t \in \R^m$ is a linear mapping from $x_t$.

We want to recurrently update hidden states $\{s_t\}_t$, where $s_t\in \RR^{m}$ is a vector that aims to summarize the information up to time $t$. 
We posit the following OCP objective for updating $s_t$: 
\begin{equation}
s_t = \argmin_{s\in \RR^m}\left \{ ||s - s_{t-1}||^2 + \beta_t ||s^\top k_t - x_t||^2 \right\}.
\label{eq:longhorn-obj}
\end{equation}
Here, $\beta_t$ controls how much new information about $x_t$ we want the model to incorporate. For instance, $\beta_t = 0$ implies $s_t = s_{t-1}$, while a large $\beta_t$ implies the model sacrifices stability for plasticity.

From a high-level perspective, \Eqref{eq:longhorn-obj} is solving an online prediction problem of learning a weight $s$ to predict $x_t$ given $k_t$ with a linear model $x_t \approx s \tt k_t$.
It is a supervised formulation of the 
\emph{associative memory} problem of 
memorize  $(k_t, x_t)$ pairs 
by learning a mapping from $k_t$ to $x_t$, such that given a key (input) $k_t$ the model can retrieve (predict) its corresponding value (label) $x_t$. The objective in \Eqref{eq:longhorn-obj} is motivated by the observation that the self-attention layer of the Transformer exhibits a form of online associative recall (often referred to as the induction head property)~\citep{olsson2022context}. This capability has been shown to underpin the model's ability to perform in-context learning~\citep{brown2020language}. To explain the connection, in-context learning refers to the model's ability, during inference, to generalize from a set of provided ${(k, x)}$ (question-answer) pairs and apply this understanding to a new question. This closely parallels associative recall, where the model retrieves relevant information from past interactions to address new inputs in a similar fashion.

Fortunately, this simple objective gives a closed-form solution for $s_t$, which coincides with the implicit online learning method~\citep[e.g.,][]{kulis2010implicit}, according to Theorem~\ref{thm:longhorn} (We provide the proof in Appendix~\ref{sec::apx-proof}):
\newline 
\begin{thm}
The closed form solution for $s_t$ for objective in \Eqref{eq:longhorn-obj} is
\begin{equation}
s_t = (I - \varepsilon_t k_t k_t^\top) s_{t-1} + \varepsilon_t k_t x_t, ~~~\text{where}~\varepsilon_t = \frac{\beta_t}{1 + \beta_t k_t^\top k_t} \in [0, \infty).
\label{eq:longhorn-closed-form}
\end{equation}
\label{thm:longhorn}
\end{thm}
As $k_t k_t^\top$ is a matrix, it is hard to compute its cumulative product for conducting a parallel scan. As a result, in practice, we use the diagonal approximation $1_m - \varepsilon_t k_t^{\odot 2}$ in place of $I - \varepsilon_t k_t k_t^\top$, where $x^{\odot 2} = x \odot x$ and $1_m$ is the $m$-dimensional all-one vector.

The above is under the simplified 1D setting. In practice, following Mamba~\citep{gu2023mamba} and Transformer~\citep{vaswani2017attention}, $x_t \in \R^d$ is a vector, and $k_t(x_t) = W_k x_t \in \R^m$ is a \emph{shared key} across $d$-dimension, which is a linear mapping from $x_t$. We similarly make $\beta(x_t) = \sigma(W_\beta x_t) \in \R^d$ a function of $x_t$, where the activation $\sigma$ (the Sigmoid function) is to ensure that $\beta(x_t)$ is positive and bounded.  As a result, $x_t, \beta_t, \varepsilon_t \in \RR^d, k_t \in \R^m$, and the memory state $S_t \in \RR^{d \times m}$ is a matrix. Then, \ours{}'s update becomes:
\begin{equation}
S_t = A_t \odot S_{t-1} + B_t, ~~\text{where}~~ A_t = (1_{d \times m} - \varepsilon_t \otimes k_t^{\odot 2} ),~~B_t = (\varepsilon_t \odot x_t) \otimes k_t.
\label{eq:longhorn-ssm-matrix}
\end{equation}
The final architecture of \ours{} follows Mamba strictly (Figure~\ref{fig:mamba-block}), except that we replace the SSM block with \ours{}'s recurrence. We also provide an efficient CUDA kernel for it. 
The full inference-time algorithm is provided in Algorithm~\ref{alg:longhorn}. One can compare \Eqref{eq:longhorn-ssm-matrix} to \Eqref{eq:mamba-ssm} and other SSMs in Appendix~\ref{sec::apx-prior-deep-ssms}. \ours{} does not introduce an extra ``forgetting" gate (hence it has fewer parameters), because the forgetting gate is naturally derived from the key vector, i.e., $(1_{d \times m} - \varepsilon_t \otimes k_t^{\odot 2})$.

\paragraph{Advantages of \ours{}} 
\begin{enumerate}
    \item While we can derive the learning objective for some of the existing SSMs, \ours{} is the first SSM designed for explicitly solving an online regression problem. 
    \item \ours{} does not require a specific forget gate (e.g., $\alpha_t$ in GLA or $A$ matrix in Mamba). The forgetting is naturally linked to the key vector $k_t$ through the derivation. This saves about $\mathcal{O}(d \times m)$ parameters per SSM module, where $m$ is the dimension of $k_t$, and $d$ is the dimension of $x_t$. However, \ours{} demonstrates better performance even with fewer parameters than Mamba (See Figure~\ref{fig:fig1} (left), Table~\ref{tab:openwebtext_scaling_law}, Table~\ref{tab:slimpajama}). 
    \item The closed-form solution in \Eqref{eq:longhorn-closed-form} \emph{does not need any specific initialization}. In contrast, Mamba requires a special careful initialization of the $A$ and $\varepsilon_t$.
    \item Unlike DeltaNet~\citep{yang2024parallelizing}, which struggles to extrapolate beyond training contexts, \ours{} successfully extrapolates to contexts \emph{16x longer} than it was trained for (Figure~\ref{fig:fig1} (right)).
\end{enumerate}
